Introduction to Renormalisation

These are introductory lecture notes aimed at beginning graduate students covering fundamental concepts and ideas behind the renormalisation group. Our main goal is to motivate it and then explore its consequences, in the context of quantum field theory. We shall reproduce the standard results without needing any mention of cancellation of infinities. To keep the story simple and compact, we'll ignore the role of symmetry in this game. We'll also restrict to scalar fields, and not mention neither fermions nor gauge fields. Moreover, we'll only briefly mention the connection with statistical field theory. Knowledge of quantum mechanics and special relativity is essential. Prior knowledge of quantum field theory is not required, however, this is not designed to be an introduction to QFT, so it may not be the most pedagogical way to introduce the topic. Previous familiarity with path integrals is also not assumed.

==> invitation.tex <==
\section{Invitation: The propagator in $\phi^4$ theory}

Historically, renormalisation appeared as a procedure to make sense of the infinities encountered in calculating contributions from Feynman\footnote{Richard Phillips Feynman (1918-1988), American, PhD supervisor: John Archibald Wheeler, Nobel prize 1965  with Julian Schwinger and Shin'ichiro Tomonaga "for their fundamental work in quantum electrodynamics (QED) with deep-ploughing consequences for the physics of elementary particles"} diagrams with loops. We shall proceed semi-historically and motivate what issues show up and how to solve them. Later we'll go back and figure why do these issues appeared and why our solution actually worked. But for now let's build intuition with the simplest possible example, calculating the propagator in $\phi^4$ theory. To recap, this is our Lagrangian\footnote{Joseph-Louis Lagrange (1736-1813), French}

\begin{equation}
    \mathcal{L}=-\frac{1}{2}\partial_\mu\phi\partial^\mu\phi-\frac{1}{2}m^2\phi^2-\frac{\lambda}{4!}\phi^4
\end{equation}

In the free theory, the only contribution to the 2-point correlation function is the propagator:

\begin{equation}
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=2cm of a] (b);
    
    \diagram* {
      (a) -- [plain,out=0,in=180, momentum=$p$] (b),
    };
  \end{feynman}
\end{tikzpicture}
    =-\frac{\ii}{p^2+m^2}
    \label{propagator}
\end{equation}

Now, in the full interacting theory, we need to include a whole series of diagrams:

\begin{equation}
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1.5cm of a] (b);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=180] (d),
      (d) -- [plain,out=0,in=45] (c),
    };
    \draw[fill=black] (c) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=0.5cm of a] (c);
    \vertex [right=0.75cm of c] (d);
    \vertex [right=0.5cm of d] (b);
    \vertex [above=1cm of c] (e);
    \vertex [above=1cm of d] (f);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (d),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=180] (e),
      (e) -- [plain,out=0,in=45] (c),
      (d) -- [plain,out=135,in=180] (f),
      (f) -- [plain,out=0,in=45] (d),
    };
    \draw[fill=black] (c) circle (1.5pt);
    \draw[fill=black] (d) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    \vertex [above=1cm of d] (e);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=-135] (d),
      (d) -- [plain,out=-45,in=45] (c),
      (d) -- [plain,out=135,in=180] (e),
      (e) -- [plain,out=0,in=45] (d),
    };
    \draw[fill=black] (c) circle (1.5pt);
    \draw[fill=black] (d) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.base)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=0.5cm of a] (c);
    \vertex [right=1cm of c] (d);
    \vertex [right=0.5cm of d] (b);
    \vertex [right=0.5cm of c] (e);
    \vertex [above=0.5cm of e] (f);
    \vertex [below=0.5cm of e] (g);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (d),
      (d) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=90,in=180] (f),
      (f) -- [plain,out=0,in=90] (d),
      (c) -- [plain,out=-90,in=180] (g),
      (g) -- [plain,out=0,in=-90] (d),
    };
    \draw[fill=black] (c) circle (1.5pt);
    \draw[fill=black] (d) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+\ldots
\end{equation}

This looks like a huge mess! But we can make some progress. For example, the third term looks like two copies of the second. This suggests we should be able to only consider "distinct" diagrams. We say that a diagram is one-particle irreducible (1PI) if it has no bridges. Where a bridge is a line that once removed makes the diagram disconnected. For example, the second is 1PI but the third isn't, because, if we remove the middle propagator, we get two disconnected diagrams (two copies of the second term). We can then write a series for the 1PI diagrams with two external legs:

\begin{equation}
\begin{tikzpicture}[baseline=(b.base)]
  \begin{feynman}
    \vertex (a);
    \vertex [blob,right=1cm of a] (c) {1PI};
    \vertex [right=1.25cm of c] (b);

    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
=
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=180] (d),
      (d) -- [plain,out=0,in=45] (c),
    };
    \draw[fill=black] (c) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    \vertex [above=1cm of d] (e);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=-135] (d),
      (d) -- [plain,out=-45,in=45] (c),
      (d) -- [plain,out=135,in=180] (e),
      (e) -- [plain,out=0,in=45] (d),
    };
    \draw[fill=black] (c) circle (1.5pt);
    \draw[fill=black] (d) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.base)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=0.5cm of a] (c);
    \vertex [right=1cm of c] (d);
    \vertex [right=0.5cm of d] (b);
    \vertex [right=0.5cm of c] (e);
    \vertex [above=0.5cm of e] (f);
    \vertex [below=0.5cm of e] (g);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (d),
      (d) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=90,in=180] (f),
      (f) -- [plain,out=0,in=90] (d),
      (c) -- [plain,out=-90,in=180] (g),
      (g) -- [plain,out=0,in=-90] (d),
    };
    \draw[fill=black] (c) circle (1.5pt);
    \draw[fill=black] (d) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+\ldots
\end{equation}

We'll call this expansion $\Pi(p^2)$ ($p$ is the external momenta, and we have amputated the two external propagators), this is often called the \textit{self-energy} of the field. Using this notation the propagator is then:

\begin{equation*}
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=2cm of a] (b);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.base)]
  \begin{feynman}
    \vertex (a);
    \vertex [blob,right=1cm of a] (c) {1PI};
    \vertex [right=1.25cm of c] (b);

    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.base)]
  \begin{feynman}
    \vertex (a);
    \vertex [blob,right=0.5cm of a] (c) {1PI};
    \vertex [blob,right=1.25cm of c] (d) {1PI};
    \vertex [right=1cm of d] (b);

    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (d),
      (d) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
+\ldots=
\end{equation*}
\vspace{-4mm}
\begin{align}
    &=-\frac{\ii}{p^2+m^2}+\frac{-\ii}{p^2+m^2}\Pi(p^2)\frac{-\ii}{p^2+m^2}+\frac{-\ii}{p^2+m^2}\Pi(p^2)\frac{-\ii}{p^2+m^2}\Pi(p^2)\frac{-\ii}{p^2+m^2}+\dots\nonumber\\
    &=-\frac{\ii}{p^2+m^2+\ii\Pi(p^2)}
\end{align}
where in going to the last line we summed the geometric series.

Looking at this expression, we can now interpret the meaning of these extra diagrams. They change the mass of the particle. Or better said, they mean that the "true" measurable mass of the particle is not the parameter we naively insert in the Lagrangian, it has contributions from the interaction terms. It's also not hard to see that these kinds of loop corrections will have the same effect over any parameter in the Lagrangian, so we'll relabel the original parameters with a subscript 0 to emphasise they are not the ones we actually measure.

\begin{equation}
    \mathcal{L}=-\frac{1}{2}\partial_\mu\phi\partial^\mu\phi-\frac{1}{2}m_0^2\phi^2-\frac{\lambda_0}{4!}\phi^4
    \label{lagrangian}
\end{equation}

Now all we're left to do is calculate $\Pi(p^2)$. To 1-loop accuracy:

\begin{equation}
    \Pi(p^2)=
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=180,momentum={[arrow shorten=0.27] $k$}] (d),
      (d) -- [plain,out=0,in=45] (c),
    };
    \draw[fill=black] (c) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
=\frac{-\ii\lambda_0}{2}\int\frac{\dd[4]{k}}{(2\pi)^4}\frac{-\ii}{k^2+m_0^2}
\end{equation}

But how the hell do we calculate that integral?? The minus sign in the Minkowski\footnote{Hermann Minkowski (1864-1909), German, PhD supervisor: Ferdinand von Lindemann} metric seems to be screwing everything up. To do it we'll use a trick (and by trick I mean cheating) called \textit{Wick\footnote{Gian Carlo Wick (1909-1992), Italian, PhD supervisor: Gleb Wataghin} rotation}. We make the transformation $k^0\to \ii k^0$, relabel $k^4=k^0$, and then rotate the contour so that we're integrating over real $k^4$. Then I say the words "analytic continuation" and point out that when you rotate the contour you don't pass through any poles so it should work. I know this sounds really unconvincing (it still does for me...) but it does work. Anyway, now it's usual Riemannian\footnote{Georg Friedrich Bernhard Riemann (1826-1866), German, PhD supervisor: Carl Friedrich Gauss} geometry so we know how to calculate it:

\begin{equation}
    \Pi(p^2)=-\frac{\ii\lambda_0}{2}\int\frac{\dd[4]{k}}{(2\pi)^4}\frac{1}{k^2+m_0^2}=-\frac{\ii\lambda_0}{2}\frac{\text{Vol}(S^3)}{(2\pi)^4}\int_0^\infty\dd{k}\frac{k^3}{k^2+m_0^2}
\end{equation}

But, for large internal momentum, the integrand goes as $\sim k$ which is divergent! This appears to say that the real mass of the particle is infinite! Which is certainly false. Our theory as defined makes no sense at all. We need to step back and understand where we might have made a mistake.

First, identify the problem. The divergence comes from the high momentum limit of the integrand, i.e. particles with arbitrarily high momentum running around the loop. Well, we could correct that by imposing a momentum cutoff, instead of integrating over all $k<\infty$ we integrate only over $k<\Lambda$.  This kind of procedure is called \textit{regularising} our theory\footnote{You may wonder if there are other ways we can regularise our theory and render these integrals finite. There are plenty of them and we'll take a look at some other procedures later on}. Computing this new integral, we have:

\begin{equation}
    \Pi(p^2)=-\frac{\ii\lambda_0}{16\pi^2}\int_0^\Lambda\dd{k}\frac{k^3}{k^2+m_0^2}=-\frac{\ii\lambda_0}{32\pi^2}\qty(\Lambda^2-m_0^2\log(1+\frac{\Lambda^2}{m_0^2}))
\end{equation}

But we can't just do this and call it a day. What is this $\Lambda$? We drape some words around it saying that it models a finite resolution in our measurement apparatus. Since we don't know what happens above a certain scale we have no right to assume our theory is still valid at those scales, and we should not integrate over them. However, it does seem rather arbitrary. A big part of these lecture notes will be devoted to motivating this procedure and to seem how natural it actually is. But for now we'll simply proceed and look at its simple consequences.

Firstly, this procedure should be considered as part of the \textit{definition} of our theory. Our original theory made a very clear prediction for the mass of the scalar, it said it was infinite. That is clearly a rubbish theory. By introducing this regulator we are changing our original theory in order to get reasonable results.

Further, since the regulator is part of the definition of our theory, every coupling in the Lagrangian is only defined at that particular value of $\Lambda$ therefore it is only natural that it should depend on $\Lambda$. But what is its exact dependence on the cutoff? Said another way, how must we change the couplings so that if we decided to use a different coupling, say $\Lambda/2$, we actually have the same physical predictions? A related question is how are the parameters in the Lagrangian, including the cutoff, related to actual experimentally measurable parameters? We'll only fully answer this questions at the end of these notes, but we'll give a quick example of how to do this.

We split the action into two pieces: the "bare" part and the "counterterm" part. We assume that the "bare" couplings do not depend on scale, all the dependence on $\Lambda$ is in the "counterterm" piece. 

\begin{align}
    S_\text{bare}&=\int\dd[4]{x}\qty{-\frac{1}{2}\partial_\mu\phi\partial^\mu\phi-\frac{1}{2}m_0^2\phi^2-\frac{\lambda_0}{4!}\phi^4}\\
    S_\text{CT}&=\int\dd[4]{x}\qty{-\frac{1}{2}\var{Z}\partial_\mu\phi\partial^\mu\phi-\frac{1}{2}\var{m}^2\phi^2-\frac{\var{\lambda}}{4!}\phi^4}
\end{align}

We have additionally included a counterterm in the gradient term since it can also, in general, receive corrections from loop diagrams. We should not assume it stays fixed at the canonical value of 1. This factor is called \textit{field strength renormalisation}\footnote{You'll also often find the name \textit{wavefunction} renormalisation in the literature, which comes from the longstanding confusion between fields and wavefunctions in quantum field theory.}. We will include the contributions from the counterterm part of the action in a funny way. Each counterterm counts as a loop, ie, for 1-loop level contributions from the "bare" action we use tree level contributions from the "counterterm" part and so on. This ensures that for each order in the perturbative expansion we only need to know what happens at lower orders in the expansion and therefore the algorithm is consistent. Ultimately this procedure is just an artifial, computational choice. No actual physics involved.

In our case the full contribution is then:

\begin{equation*}
\Pi(p^2)=
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [right=1cm of a] (c);
    \vertex [right=1cm of c] (b);
    \vertex [above=1cm of c] (d);
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
      (c) -- [plain,out=135,in=180] (d),
      (d) -- [plain,out=0,in=45] (c),
    };
    \draw[fill=black] (c) circle (1.5pt);
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [crossed dot,right=0.75cm of a] (c) {};
    \vertex [right=1cm of c] (b);
    \vertex [above=0.45cm of c] (d) {$\ii p^2\var{Z}$};
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
+
\begin{tikzpicture}[baseline=(b.south)]
  \begin{feynman}
    \vertex (a);
    \vertex [crossed dot,right=0.75cm of a] (c) {};
    \vertex [right=1cm of c] (b);
    \vertex [above=0.45cm of c] (d) {$-\ii\var{m}^2$};
    
    \diagram* {
      (a) -- [plain,out=0,in=180] (c),
      (c) -- [plain,out=0,in=180] (b),
    };
  \end{feynman}
\end{tikzpicture}
=
\end{equation*}

\begin{equation}
    =-\frac{\ii\lambda_0}{32\pi^2}\qty(\Lambda^2-m_0^2\log(1+\frac{\Lambda^2}{m_0^2}))+\ii p^2\var{Z}-\ii\var{m}^2
\end{equation}

We now need to fix the counterterms. Using our knowledge of scattering amplitudes we know that the propagator should have a pole at $p^2=m_\text{phys}^2$ and that that pole should be simple, this allows us to figure out which is the actual physical mass. We then fix the counterterms such that this is true. These kinds of choices are called \textit{renormalisation schemes}, this one in particular is the \textit{on-shell} scheme. It gives us the following two requirements which allow us to fix both $\var{Z}$ and $\var{m}^2$.

\begin{align}
    m_\text{phys}^2-m_0^2-\ii\Pi(-m_\text{phys}^2)=0\\
    \eval{\pdv{\Pi}{p^2}}_{p^2=-m_\text{phys}^2}=0
\end{align}

The second one gives $\var{Z}=0$, the first one gives

\begin{equation}
    \var{m}^2=m_0^2-m_\text{phys}^2-\frac{\lambda_0}{32\pi^2}\qty(\Lambda^2-m_0^2\log(1+\frac{\Lambda^2}{m_0^2}))
\end{equation}

We still have to choose the value of $m_0$, we make the simple choice $m_0=m_\text{phys}=m$ so that,

\begin{equation}
    \var{m}^2=-\frac{\lambda_0}{32\pi^2}\qty(\Lambda^2-m^2\log(1+\frac{\Lambda^2}{m^2}))
\end{equation}

Well this seemed like a useless exercise. We did some difficult integrals, made several changes of notation and ended up with a propagator that looks like (\ref{propagator}). There are two things we must note however, firstly, this was a \textit{very} simple example, it was a mere accident that there was no dependence on the external momentum, and that simplified our analysis a lot, in more complicated examples we would not have such a simple calculation. 

Further, this result is not simple at all, because our mass coupling is \textit{not} $\frac{1}{2}m^2\phi^2$, it is $$\frac{1}{2}(m^2+\var{m}^2)\phi^2=\frac{1}{2}\qty(m^2-\frac{\lambda_0}{32\pi^2}\qty(\Lambda^2-m^2\log(1+\frac{\Lambda^2}{m^2})))\phi^2$$and it was through our mighty 1-loop integrals that we could understand what that meant. However, the way we managed to "remove" the infinities and extract physically meaningful results is, as Feynman put it, a "dippy process". To fully understand what have we actually done why do we need to do it we must change into the path integral formulation of quantum field theory.

\newpage

